Collision Cascade-Driven Evolution of Vacancy Defects in Ni-Based Concentrated Solid-Solution Alloys

Concentrated solid--solution alloys (CSAs) in single--phase form have recently garnered considerable attention owing to their potential for exceptional irradiation resistance. This computational study delves into the intricate interplay of alloying elements on the generation, recombination, and evolution of irradiation-induced defects. Molecular dynamics simulations were conducted for collision cascades at room temperature, spanning a range of primary knock-on atom energies from 1 to 10 keV. The investigation encompasses a series of model crystals, progressing from pure Ni to binary CSAs such as NiFe$_{20}$, NiFe, NiCr$_{20}$, and culminating in the more intricate NiFeCr$_{20}$ CSA. We observe that materials rich in chromium actively facilitate dislocation emissions and induce the nucleation of stacking fault tetrahedra in the proximity of nanovoids, owing to Shockley partial interactions. This result is validated by molecular static simulations, which calculate the surface, vacancy, and defect formation energies. Among various shapes considered, the spherical void proves to be the most stable, followed by the truncated octahedron and octahedron shapes. On the other hand, the tetrahedron cubic shape is identified as the most unstable, and stacking fault tetrahedra exhibit the highest formation energy. Notably, among the materials studied, NiCr$_{20}$ and NiFeCr$_{20}$ CSAs stood out as the sole alloys capable of manifesting this mechanism, mainly observed at high impact energies.

==> sections/methods_2.tex <==
\section{Computational methods}
\label{sec:methods}
%\subsection{Interatomic potential}

The atomistic behavior of the samples was modeled using the 
Molecular Dynamics method with interatomic potentials based on 
the embedded atom model (EAM) to describe atom-to-atom interactions \cite{BONNY201742,Bonny_2013}. 
The Large-scale Atomic Molecular Massively Parallel Simulator (LAMMPS) 
\cite{THOMPSON2022108171}
was employed for this purpose.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

composition
randomness of CSA

Methodology to calculate elastic constants
Methodology to calculate GSF energy
Methodology for creation of SFT and voids, and calculation of formation energies

-> size cell / static minimization procedure for the three previous

Methodology for displacement cascades
               Size cell / MD procedure (what is the pka?)
               
Analysis (defects, voids and dislocations)

Section: Properties of the Bulk
               -cell parameter
               -bulk modulus
Section: stability of defects
-        GSF
-        SFT and voids

\subsection{GSF method}
For the computation of the Generalized Stacking Fault (GSF) energy, a numerical
cell with the orientation of $X=[1 \Bar{1} 0]$, $Y=[1 1 \Bar{2}]$, and $Z=[111]$
and dimensions $(d_x, d_y, d_z) = (2.5, 2.5, 9)$ nm was utilized.
Periodic boundary conditions were implemented in the $X$ and $Y$ directions,
while free surfaces were allowed in the $Z$ direction. 
Solute atoms were uniformly and randomly distributed across 10 different 
samples following the same atomic percentages for the CSAs
to ensure a reliable average of the GSF energy, denoted as $\gamma_{\rm GSF}$.
The stacking fault was introduced by rigidly shifting the half upper region 
of the cell in the $X$ and $Y$ directions. Subsequent relaxation of the cell
occurred until the interatomic force reached 0.1 meV/\AA.
The energy of the cell, denoted as $E_{\rm GSF}$, was then computed based
on the displacement of the cell in the $Y$ direction.% (Fig. \ref{fig:GSF}).
\begin{equation}
    \gamma_{GSF} = \frac{E_{\rm GSF}-E_0}{A}
\end{equation}
with $E_0$ the energy of the cell without the stacking fault, $i.e$. without any
shift, and $A$ is the GSF area. 


\subsection{Stacking Fault Tetrahedra}

We build simulation cells to study the solid--solution alloys and
the pure Ni crystal oriented in the $[001]$ direction. 
The simulation involved $N_{at} \simeq 863 000$ atoms, arranged
within dimensions $(d_x, d_y, d_z)$ = (21, 21, 21) nm. 
Our investigation focused on various alloys, namely NiFe, NiFe$_{20}$, 
NiCr$_{20}$, and NiFeCr$_{20}$ which were compared to pure Ni case.
Solute atoms were randomly introduced by substituting pure crystal
Ni atoms. To account for randomness, computations were conducted
across 10 different random alloy configurations.
It is well--established that defects in fcc metals exhibit
diverse shapes and characteristics \cite{eyre1973transmission}. 
Particularly, vacancy clusters and stacking fault tetrahedra are 
prominently observed defects in these fcc metals
\cite{chakraborty2017cr}. 

\subsection{Voids}
We build void of spherical, octahedron and truncated octahedron
(as predicted by wulff theory, see Fig. \ref{fig:wulff}),
tetrahedron and cubic shapes. 
Stacking fault tetrahedra (SFT) were introduced using
the method outlined in this work Ref. \cite{kadoyoshi2007molecular}.
\begin{figure}[b!]
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/wulff.png}
    \caption{Wulff shape predictions computed based on the surface energy of alloys (refer to the supplementary material for details) \cite{marks1983modified,wul1901frage}.}
    \label{fig:wulff}
\end{figure}
The mean formation energy per vacancy, $E_f$, of these defects was merely computed as follows:
\begin{equation}
    E_f = \frac{1}{N_{at} - N_d} \left( E_{d} - \frac{N_d}{N_{at}} E_0 \right)
\end{equation}
where $E_d$ is the energy of the simulation cell with the defect, 
containing $N_d$ atoms and $N_{at}-N_d$ vacancy and $E_0$ is the energy of 
the simulation cell of the pristine crystal, containing $N_{at}$ atoms. We 
choose to rationalize the formation energy over the number of vacancies 
since, defects of same size can have different number of vacancies due to 
their peculiar shape. 
